SpeechCLIP: Integrating Speech with Pre-Trained Vision and Language Model

Data-driven speech processing models usually perform well with a large amount of text supervision, but collecting transcribed speech data is costly. Therefore, we propose SpeechCLIP, a novel framework bridging speech and text through images to enhance speech models without transcriptions. We leverage state-of-the-art pre-trained HuBERT and CLIP, aligning them via paired images and spoken captions with minimal fine-tuning. SpeechCLIP outperforms prior state-of-the-art on image-speech retrieval and performs zero-shot speech-text retrieval without direct supervision from transcriptions. Moreover, SpeechCLIP can directly retrieve semantically related keywords from speech.

==> figure/ks_weight_small.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{figure/hidden_weights/asr_large_coco_weights.pdf}
    \vspace{-16pt}
    \caption{
        Normalized weights for layer summarization of \hubert  and \speechclip in SUPERB ASR task.
        \texttt{CNN} and \texttt{Trm} respectively denote the \hubert CNN feature extractor and the transformer encoder layer in \speechclip.
    }
    \label{fig:ks_weight_small}
\end{figure}


==> figure/layer_weights_SUPERB.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth,trim={0.2cm 0cm 0.2cm 0cm},clip]{figure/layer_weights_SUPERBJS.pdf}
    \vspace{-20pt}
    \caption{
        The heatmap shows the JS divergence of learned weights for weighted sum of hidden layers between \speechclip's speech encoder pre-trained on \flickr and \hubert Base trained on SUPERB~\cite{yang2021superb} tasks.
    }
    \label{fig:superb_layer_weights}
\end{figure}


==> figure/model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figure/KWCLIP-Cacaded.pdf}
    \caption{\jeff{Testing figure size}}
    \label{fig:model}
\end{figure}


==> table/pr_asr.tex <==
\begin{table}[t]
    \caption{
        \textbf{PR} and \textbf{ASR} results of \speechclip models trained with \flickr.
        The metrics are phoneme error rate (PER\%) and word error rate (WER\%).
        Subscripts for ASR indicate the vocabulary type, where char denotes character, and 1k denote the subword vocabulary size.
    }
    % \vspace{2pt}
    \label{tab:pr_asr}
    \centering
    \small
    % \footnotesize
    \begin{tabular}{@{~~}l@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~} }
        \toprule
        & PR & ASR$_{\text{char}}$ & ASR$_{\text{1k}}$ \\
        \cmidrule{2-4}
        Method & PER$\downarrow$ & WER$\downarrow$ &  WER$\downarrow$ \\
        \midrule
        HuBERT Base  & 5.41 & 6.42 & 6.17  \\
        FaST-VGS+ & 7.76 & 8.83 & 8.22 \\
        \midrule
        Parallel & 4.95 & 6.46 & 6.24 \\
        Cascaded & \textbf{4.92} & \textbf{6.34} & \textbf{6.15}  \\
        \bottomrule
    \end{tabular}
    % \vspace{-8pt}
\end{table}


==> table/superb.tex <==
\begin{table*}[t]
    \caption{
        Results on SUPERB \cite{yang2021superb}.
        The metrics include accuracy (Acc\%) phoneme error rate (PER\%), word error rate (WER\%), F1 score (F1\%), and concept error rate (CER\%).
        LS960, LL60k, Mix94k, and YFCC15M respectively denote LibriSpeech 960 hr corpus~\cite{Panayotov2015libri}, Libri-Light 60k hr corpus~\cite{kahn2020libri}, Mix 94k hr corpus~\cite{chen2021wavlm}, and the subset of YFCC100M used for CLIP pre-training~\cite{thomee2016yfcc100m}.
        % Subscripts for ASR tasks indicate the vocabulary type, where char denotes character-based ASR as SUPERB does, while 300 and 1k denotes the size of subword vocabulary.
    }
    % \vspace{2pt}
    \label{tab:superb}
    \centering
    \small
    % \footnotesize
    \begin{tabular}{@{~~}l@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~~}c@{~~}c@{~~~}c@{~~}}
        \toprule
        &  &  & \multicolumn{3}{c}{Content} &  & \multicolumn{2}{c}{Semantics} \\
        \cmidrule{4-6}
        \cmidrule{8-9}
        &  &  &  PR & ASR & KS & & IC & SF \\
        \cmidrule{4-9}
        Method & \hl{\# Param.} & Data & PER$\downarrow$ & WER$\downarrow$ & Acc$\uparrow$ &  & Acc$\uparrow$ & F1$\uparrow$ / CER$\downarrow$ \\
        \midrule
        \multicolumn{3}{l}{\textit{Speech SSL Baselines}} \\
        \midrule
        HuBERT Base & 94.68M & LS960 & 5.41 & 6.42 & 96.30 & & 98.34 & 88.53 / 25.20 \\
        HuBERT Large & 316.61M & LL60k & 3.53 & 3.62 & 95.29 & & 98.76 & 89.81 / 21.76 \\
        WavLM Large & 316.62M & Mix94k & 3.06 & 3.44 & 97.86 & & 99.31 & 92.21 / 18.86 \\
        \midrule
        \multicolumn{3}{l}{\textit{Visually Enhanced Speech SSL}} \\
        \midrule
        FaST-VGS & 187.87M & LS960 + \coco & 16.30 & 13.46 & 96.85 & & 98.37 & 84.91 / 32.33 \\
        FaST-VGS+ & 217.23M & LS960 + \coco & 7.76 & 8.83 & 97.27 & & 98.97 & 88.15 / 27.12 \\
        \midrule
        \multicolumn{3}{l}{\textit{SpeechCLIP (Ours)}} \\
        \midrule
        Parallel &  & LS960 + YFCC15M + \flickr & 4.95 & 6.46 & 96.56 &  & 97.71 &	88.23 /	24.93 \\
        Cascaded &  & LS960 + YFCC15M + \flickr & 4.92 & 6.34 & 96.62 &  & 98.02 &	88.90 /	23.28 \\
        % Hybrid &  & LS960 + YFCC15M + Flickr & 4.98 &	6.47 & \hl{6.21} & 6.23  & 96.59 &  & 98.15&	88.26/	25.04 \\
        \midrule
        Parallel Large &  & LL60k + YFCC15M + \flickr & 2.94 & 3.68 & 95.68 &    &  98.50  & 89.18 / 22.38 \\
        Cascaded Large &  & LL60k + YFCC15M + \flickr & 2.98 & 3.66 & 95.62 &    & 98.52 & 88.64 / 22.90  \\
        % Hybrid Large &  & LL60k + YFCC15M + Flickr & 3.01  & 3.74  &  &  & 95.62 &  &  98.60  & 89.65 / 21.82  \\
        \midrule
        Parallel Large &     & LL60k + YFCC15M + \coco & 2.89 & 3.66 & 95.62 &  & 98.73  & 88.92 / 22.04 \\
        Cascaded Large &    & LL60k + YFCC15M + \coco & 2.97 & 3.68 & 95.62 & & 98.52 & 89.13 / 22.11 \\
        % Hybrid Large &     & LL60k + YFCC15M + SC & 3.00 & 3.60  &  &  & 95.42 &  & 98.68  & 88.98 / 22.77  \\
        \bottomrule
    \end{tabular}
    \vspace*{-8pt}
\end{table*}


==> table/superb_old.tex <==
\begin{table*}[t]
    \caption{
        Results on SUPERB \cite{yang2021superb}.
        The metrics include accuracy (Acc\%) phoneme error rate (PER\%), word error rate (WER\%), F1 score (F1\%), and concept error rate (CER\%).
        % Subscripts for ASR tasks indicate the vocabulary type, where char denotes character-based ASR as SUPERB does, while 300 and 1k denotes the size of subword vocabulary.
    }
    \vspace{2pt}
    \label{tab:superb}
    \centering
    \small
    % \footnotesize
    \begin{tabular}{@{~~}l@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~}c@{~}c@{~~}c@{~~}}
        \toprule
        &  &  & \multicolumn{5}{c}{Content} &  & \multicolumn{2}{c}{Semantics} \\
        \cmidrule{4-8}
        \cmidrule{10-11}
        &  &  &  PR & ASR$_{\text{char}}$ & ASR$_{\text{300}}$ & ASR$_{\text{1k}}$ & KS & & IC & SF \\
        \cmidrule{4-11}
        Method & \# Param. & Data & PER$\downarrow$ & WER$\downarrow$ & WER$\downarrow$ & WER$\downarrow$ & Acc$\uparrow$ &  & Acc$\uparrow$ & F1$\uparrow$ / CER$\downarrow$ \\
        \midrule
        \multicolumn{3}{l}{\textit{Speech SSL Baselines}} \\
        \midrule
        HuBERT Base & 94.68M & LS960 & 5.41 & 6.42 &  &  & 96.30 & & 98.34 & 88.53 / 25.20 \\
        HuBERT Large & 316.61M & LL60k & 3.53 & 3.62 &  &  & 95.29 & & 98.76 & 89.81 / 21.76 \\
        WavLM Large & 316.62M & Mix94k & 3.06 & 3.44 &  &  & 97.86 & & 99.31 & 92.21 / 18.86 \\
        \midrule
        \multicolumn{3}{l}{\textit{Visually Enhanced Speech SSL}} \\
        \midrule
        FaST-VGS & 187.87M & LS960 + SC & 16.30 & 13.46 / 9.51 &  &  & 96.85 & & 98.37 & 84.91 / 32.33 \\
        FaST-VGS+ & 217.23M & LS960 + SC & 7.76 & 8.83 / 6.37 &  &  & 97.27 & & 98.97 & 88.15 / 27.12 \\
        \midrule
        \multicolumn{3}{l}{\textit{SpeechCLIP (Ours)}} \\
        \midrule
        Parallel &  & LS960 + YFCC15M + Flickr   & 4.95 &	6.46 & 6.22 & 6.24 & 96.56 &  & 97.71 &	88.23 /	24.93 \\
        Cascaded &  & LS960 + YFCC15M + Flickr & 4.92 & 6.34 & 6.18 & 6.15 & 96.62 &  & 98.02 &	88.90 /	23.28 \\
        % Hybrid &  & LS960 + YFCC15M + Flickr & 4.98 &	6.47 & \hl{6.21} & 6.23  & 96.59 &  & 98.15&	88.26/	25.04 \\
        \midrule
        Parallel Large &  & LL60k + YFCC15M + Flickr & 2.94 & 3.68 &  &  & 95.68 &    &  98.50  & 89.18 / 22.38 \\
        Cascaded Large &  & LL60k + YFCC15M + Flickr & 2.98 & 3.66 &  &  & 95.62 &    & 98.52 & 88.64 / 22.90  \\
        % Hybrid Large &  & LL60k + YFCC15M + Flickr & 3.01  & 3.74  &  &  & 95.62 &  &  98.60  & 89.65 / 21.82  \\
        \midrule
        Parallel Large &     & LL60k + YFCC15M + SC & 2.89 & 3.66 &  &  & 95.62 &  & 98.73  & 88.92 / 22.04 \\
        Cascaded Large &    & LL60k + YFCC15M + SC & 2.97 & 3.68 &  &  & 95.62 & & 98.52 & 89.13 / 22.11 \\
        % Hybrid Large &     & LL60k + YFCC15M + SC & 3.00 & 3.60  &  &  & 95.42 &  & 98.68  & 88.98 / 22.77  \\
        \bottomrule
    \end{tabular}
    \vspace*{-8pt}
\end{table*}

